Journey to the Center of Software Supply Chain Attacks

This work discusses open-source software supply chain attacks and proposes a general taxonomy describing how attackers conduct them. We then provide a list of safeguards to mitigate such attacks. We present our tool "Risk Explorer for Software Supply Chains" to explore such information and we discuss its industrial use-cases.

==> ReferencesAnalysis/all-refs-years.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=23.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23},
xticklabel style={rotate=90.0},
xticklabels={
  1984.0,
  1999.0,
  2002.0,
  2003.0,
  2004.0,
  2005.0,
  2006.0,
  2007.0,
  2008.0,
  2009.0,
  2010.0,
  2011.0,
  2012.0,
  2013.0,
  2014.0,
  2015.0,
  2016.0,
  2017.0,
  2018.0,
  2019.0,
  2020.0,
  2021.0,
  2022.0,
  2023.0
},
y grid style={darkgray176},
ymin=0, ymax=75.6,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.25,0) rectangle (axis cs:0.25,1);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180}
\addlegendentry{year}

\draw[draw=none,fill=steelblue31119180] (axis cs:0.75,0) rectangle (axis cs:1.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:1.75,0) rectangle (axis cs:2.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:2.75,0) rectangle (axis cs:3.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:3.75,0) rectangle (axis cs:4.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:4.75,0) rectangle (axis cs:5.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:5.75,0) rectangle (axis cs:6.25,3);
\draw[draw=none,fill=steelblue31119180] (axis cs:6.75,0) rectangle (axis cs:7.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:7.75,0) rectangle (axis cs:8.25,3);
\draw[draw=none,fill=steelblue31119180] (axis cs:8.75,0) rectangle (axis cs:9.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:9.75,0) rectangle (axis cs:10.25,10);
\draw[draw=none,fill=steelblue31119180] (axis cs:10.75,0) rectangle (axis cs:11.25,5);
\draw[draw=none,fill=steelblue31119180] (axis cs:11.75,0) rectangle (axis cs:12.25,3);
\draw[draw=none,fill=steelblue31119180] (axis cs:12.75,0) rectangle (axis cs:13.25,8);
\draw[draw=none,fill=steelblue31119180] (axis cs:13.75,0) rectangle (axis cs:14.25,9);
\draw[draw=none,fill=steelblue31119180] (axis cs:14.75,0) rectangle (axis cs:15.25,12);
\draw[draw=none,fill=steelblue31119180] (axis cs:15.75,0) rectangle (axis cs:16.25,15);
\draw[draw=none,fill=steelblue31119180] (axis cs:16.75,0) rectangle (axis cs:17.25,26);
\draw[draw=none,fill=steelblue31119180] (axis cs:17.75,0) rectangle (axis cs:18.25,42);
\draw[draw=none,fill=steelblue31119180] (axis cs:18.75,0) rectangle (axis cs:19.25,41);
\draw[draw=none,fill=steelblue31119180] (axis cs:19.75,0) rectangle (axis cs:20.25,40);
\draw[draw=none,fill=steelblue31119180] (axis cs:20.75,0) rectangle (axis cs:21.25,72);
\draw[draw=none,fill=steelblue31119180] (axis cs:21.75,0) rectangle (axis cs:22.25,45);
\draw[draw=none,fill=steelblue31119180] (axis cs:22.75,0) rectangle (axis cs:23.25,6);
\end{axis}

\end{tikzpicture}


==> ReferencesAnalysis/attack-refs-years.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=12.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12},
xticklabel style={rotate=90.0},
xticklabels={
  2010.0,
  2011.0,
  2012.0,
  2014.0,
  2015.0,
  2016.0,
  2017.0,
  2018.0,
  2019.0,
  2020.0,
  2021.0,
  2022.0,
  2023.0
},
y grid style={darkgray176},
ymin=0, ymax=23.1,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.25,0) rectangle (axis cs:0.25,2);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180}
\addlegendentry{year}

\draw[draw=none,fill=steelblue31119180] (axis cs:0.75,0) rectangle (axis cs:1.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:1.75,0) rectangle (axis cs:2.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:2.75,0) rectangle (axis cs:3.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:3.75,0) rectangle (axis cs:4.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:4.75,0) rectangle (axis cs:5.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:5.75,0) rectangle (axis cs:6.25,5);
\draw[draw=none,fill=steelblue31119180] (axis cs:6.75,0) rectangle (axis cs:7.25,14);
\draw[draw=none,fill=steelblue31119180] (axis cs:7.75,0) rectangle (axis cs:8.25,11);
\draw[draw=none,fill=steelblue31119180] (axis cs:8.75,0) rectangle (axis cs:9.25,5);
\draw[draw=none,fill=steelblue31119180] (axis cs:9.75,0) rectangle (axis cs:10.25,14);
\draw[draw=none,fill=steelblue31119180] (axis cs:10.75,0) rectangle (axis cs:11.25,22);
\draw[draw=none,fill=steelblue31119180] (axis cs:11.75,0) rectangle (axis cs:12.25,2);
\end{axis}

\end{tikzpicture}


==> ReferencesAnalysis/peerrev-refs-years.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-0.5, xmax=19.5,
xtick style={color=black},
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19},
xticklabel style={rotate=90.0},
xticklabels={
  1999.0,
  2002.0,
  2004.0,
  2005.0,
  2006.0,
  2008.0,
  2009.0,
  2010.0,
  2011.0,
  2012.0,
  2013.0,
  2014.0,
  2015.0,
  2016.0,
  2017.0,
  2018.0,
  2019.0,
  2020.0,
  2021.0,
  2022.0
},
y grid style={darkgray176},
ymin=0, ymax=21,
ytick style={color=black}
]
\draw[draw=none,fill=steelblue31119180] (axis cs:-0.25,0) rectangle (axis cs:0.25,1);
\addlegendimage{ybar,ybar legend,draw=none,fill=steelblue31119180}
\addlegendentry{year}

\draw[draw=none,fill=steelblue31119180] (axis cs:0.75,0) rectangle (axis cs:1.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:1.75,0) rectangle (axis cs:2.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:2.75,0) rectangle (axis cs:3.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:3.75,0) rectangle (axis cs:4.25,3);
\draw[draw=none,fill=steelblue31119180] (axis cs:4.75,0) rectangle (axis cs:5.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:5.75,0) rectangle (axis cs:6.25,2);
\draw[draw=none,fill=steelblue31119180] (axis cs:6.75,0) rectangle (axis cs:7.25,3);
\draw[draw=none,fill=steelblue31119180] (axis cs:7.75,0) rectangle (axis cs:8.25,3);
\draw[draw=none,fill=steelblue31119180] (axis cs:8.75,0) rectangle (axis cs:9.25,1);
\draw[draw=none,fill=steelblue31119180] (axis cs:9.75,0) rectangle (axis cs:10.25,6);
\draw[draw=none,fill=steelblue31119180] (axis cs:10.75,0) rectangle (axis cs:11.25,4);
\draw[draw=none,fill=steelblue31119180] (axis cs:11.75,0) rectangle (axis cs:12.25,8);
\draw[draw=none,fill=steelblue31119180] (axis cs:12.75,0) rectangle (axis cs:13.25,6);
\draw[draw=none,fill=steelblue31119180] (axis cs:13.75,0) rectangle (axis cs:14.25,9);
\draw[draw=none,fill=steelblue31119180] (axis cs:14.75,0) rectangle (axis cs:15.25,15);
\draw[draw=none,fill=steelblue31119180] (axis cs:15.75,0) rectangle (axis cs:16.25,13);
\draw[draw=none,fill=steelblue31119180] (axis cs:16.75,0) rectangle (axis cs:17.25,20);
\draw[draw=none,fill=steelblue31119180] (axis cs:17.75,0) rectangle (axis cs:18.25,17);
\draw[draw=none,fill=steelblue31119180] (axis cs:18.75,0) rectangle (axis cs:19.25,9);
\end{axis}

\end{tikzpicture}

